Qudit lattice surgery

We observe that lattice surgery, a model of fault-tolerant qubit computation, generalises straightforwardly to arbitrary finite-dimensional qudits. The generalised model is based on the group algebras $\mathbb{C}\mathbb{Z}_d$ for $d \geq 2$. It still requires magic state injection for universal quantum computation. We relate the model to the ZX-calculus, a diagrammatic language based on Hopf-Frobenius algebras.

==> biblio2.tex <==

\begin{thebibliography}{99}
\bibitem{Aaronson}S. Aaronson, Quantum computing, postselection, and probabilistic polynomial-time, Proc. R. Soc. A. 461 (2005) 3473-–3482
\bibitem{AA}A. Alekseev, H. Grosse and V. Schomerus, Combinatorial quantization of the Hamiltonian Chern--Simons theory II. Commun. Math. Phys. 174 (1996) 561--604
\bibitem{AM}N. Andruskiewitsch and J.M. Mombelli,On module categories over finite-dimensional Hopf algebras, Journal of Algebra 314(1) (2007) 383--418
\bibitem{AYY}A. Bullivant, Y. Hu, Y. Wan, Twisted Quantum Double Model of Topological Orders with Boundaries, Phys. Rev. B 96 (2017)
\bibitem{AziMa}R. Aziz and S. Majid, Codouble bosonisation and dual bases of $c_q[SL_2]$ and $c_q[SL_3]$, J. Algebra 518 (2019) 75--118 
\bibitem{Kir}B. Balsam and A. Kirillov, Jr.,  Kitaev's lattice model and Turaev-Viro TQFTs, arXiv:1206.2308
\bibitem{BGM}E. Beggs, J. Gould and S. Majid, Finite group factorisations and braiding, J. Algebra 181 (1996) 112--151
\bibitem{BSW}S. Beigi, P. Shor and D. Whalen, The quantum double model with boundary: condensations and symmetries, Comm. Math. Phys. 306 (2011) 663--694
\bibitem{Bom}H. Bombin and M. A. Martin-Delgado, Family of non-Abelian Kitaev models on a lattice: Topological condensation and confinement, Phys. Rev. B 78 (2008) 115421
\bibitem{BO}R. Bezrukavnikov and V. Ostrik, On tensor categories attached to cells in affine Weyl groups II, arXiv:math/0102220 [math.RT]
\bibitem{Cirac}G.K. Brennen, M. Aguado and J.I. Cirac, Simulations of quantum double models, New J. Phys. 11 053009
\bibitem{BMCA}O. Buerschaper, J.M. Mombelli,  M. Christandl and M. Aguado, A hierarchy of topological tensor network states, J. Math. Phys.  54 (2013) 012201
\bibitem{Chen}P. Chen, S. Cui and B. Yan, Ribbon operators in the generalized Kitaev quantum double model based on Hopf algebras, arXiv:2105.08202 [cond-mat.str-el]
\bibitem{CD}B. Coecke and R. Duncan, Interacting quantum observables: categorical algebra and diagrammatics, New J. Phys. 13 (2011) 
\bibitem{CoD}J Collins and R. Duncan, Hopf-Frobenius algebras and a simpler Drinfeld double, in eds. B. Coecke and M. Leifer, {\em Quantum Physics and Logic} 2019, EPTCS  318 (2020)150--180
\bibitem{Cui}S. Cui, D. Ding, X. Han, G. Penington, D. Ranard, B Rayhaun and Z. Shangnan, Kitaev's quantum double model as an error correcting code, Quantum 4 (2020) 331--356
\bibitem{Cui2}S. Cui, S. Hong and Z. Wang, Universal quantum computation with weakly integral anyons, Quantum Inf Process 14 (2015) 2687-–2727
\bibitem{Dri}V.G. Drinfeld, Quantum groups, in Proc. ICM Berkeley. AMS, 1987
\bibitem{tess} A. L. Edmonds and J. H. Ewing and R. S. Kulkarni, Regular Tessellations of Surfaces and (p, q, 2)-Triangle Groups, Annals of Mathematics 116 (1982) 113--132
\bibitem{Fer} 
M.J.B. Ferreira, P. Padmanabhan and P. Teotonio-Sobrinho, 2D quantum double models from a 3D perspective, J. Phys. A: Math. Theor. 47 (2014) 375204 (50pp)
\bibitem{FMMC}A. G. Fowler, M. Mariantoni, J. M. Martinis, A. N. Cleland, Surface codes: Towards practical large-scale quantum computation, Phys. Rev. A 86 (2012)
\bibitem{IH}I. Hofstetter, Extensions of Hopf algebras and their cohomological description, Journal of Algebra 164 (1994) 264--298
\bibitem{HFDM}C. Horsman, A. G. Fowler, S. Devitt, R. van Meter, Surface code quantum computing by lattice surgery, New J. Phys. 14 123011
\bibitem{Kit}A. Kitaev, Fault-tolerant quantum computation by anyons, Ann. Phys.  303 (2003) 3--20
\bibitem{KL}E. Knill and R. Laflamme, A theory of quantum error correcting codes, Phys. Rev. Lett. 84 (2000) 2525--2528
\bibitem{Kup}G. Kuperberg,  Involutory Hopf algebras and 3-manifold invariants, Int. J. Math. 2 (1991), 41--66
\bibitem{Sim}Xi-W. Luo, Y-J. Han, G-C. Guo, X. Zhou and Z-W. Zhou, Simulation of non-Abelian anyons using ribbon operators connected to a common base site, Phys. Rev. A 84 (2011) 052314
\bibitem{Ma:phy}S. Majid, Physics for algebraists: non-commutative and non-cocommutative Hopf algebras by a bicrossproduct construction, J. Algebra 130 (1990) 17--64
\bibitem{Ma:book}S. Majid, {\em Foundations of Quantum Group Theory},  Cambridge University Press, (1995); paperback  ed. (2000)
\bibitem{Ma:pri}S. Majid, {\em A Quantum Groups Primer}, L.M.S. Lect. Notes 292 (2002)
\bibitem{Ma:dg}S. Majid,  Classification of differentials on quantum doubles and finite noncommutative geometry, Lect. Notes Pure Appl. Maths 239 (2004) 167-188, Marcel Dekker
\bibitem{Ma:fro}S. Majid, Quantum and braided ZX-calculus, arXiv: 2103.07264 [math.qa]
\bibitem{Ma:rep}S. Majid, Representations, duals and quantum doubles of monoidal categories, Proceedings of the Winter School "Geometry and Physics" (1991) 197--206
\bibitem{Mas}A. Masuoka, Semisimple Hopf algebras of dimension 6, 8, Israel Journal of Mathematics (1995)
\bibitem{MD}A. Masuoka and Y. Doi, Generalization of cleft comodule algabras, Commun. in Alg. 20:12 (1992) 3703--3721
\bibitem{Meu}C. Meusburger, Kitaev lattice models as a Hopf algebra gauge theory, Commun. Math. Phys. 353 (2017) 413--468
\bibitem{Niel}M. Nielsen and I. Chuang, Quantum Computation and Quantum Information: 10th Anniversary Edition (2010), doi:10.1017/CBO9780511976667
\bibitem{Sch} H.-J. Schneider, Lectures on Hopf algebras; Notes by Sonia Natale, Trabajos de Matematica 31/95, FaMAF, 1995.
\bibitem{Tak}M. Takeuchi,  Matched pairs of groups and bismash products of Hopf algebras, Comm. Algebra 9 (1981) 841
\bibitem{fib}S. Trebst, M. Troyer, Z. Wang and A. Ludwig,  A short introduction to Fibonacci anyon models, Prog. Theor. Phys. Suppl. 176 (2008) 384--407
\bibitem{Woot}J. R. Wootton, V. Lahtinen and J. K. Pachos, Universal quantum computation with a non-Abelian topological memory, in {\em Theory of Quantum Computation, Communication, and Cryptography} (2009) 56--65
\bibitem{BM}O. Buerschaper and M. Aguado, Mapping Kitaev's quantum double lattice models to Levin and Wen's string-net models, Phs. Rev. B 80 (2009) 155136
\bibitem{CCW}I. Cong, M. Cheng and Z. Wang, Topological Quantum Computation with Gapped Boundaries, arXiv:1609.02037 [quant-ph]
\bibitem{Chang}L. Chang, Kitaev models based on unitary quantum groupoids, J. Math. Phys. 55 (2014) 041703
\bibitem{Cow}A. Cowtan and S. Majid, Quantum double aspects of surface code models, arxiv:2107.04411 [quant-ph]
\bibitem{Kir2}A. Kirillov, String-net model of Turaev-Viro invariants, arXiv:1106.6033 [math.AT]
\bibitem{KK}A. Kitaev and L. Kong, Models for Gapped Boundaries and Domain Walls, Commun. Math. Phys. 313 (2012) 351-–373
\bibitem{Kong}Liang Kong, Anyon condensation and tensor categories, Nuclear Physics B 886 (2014) 436--482
\bibitem{LW} M. Levin and X. G. Wen, String-net condensation: A physical mechanism for topological phases, Phys. Rev. B 71 (2005) 045110
\bibitem{Os}V. Ostrik, Module categories, weak Hopf algebras and modular invariants, Transform. Groups 8 (2003) 177–-206
\bibitem{NV}D. Nikshych and L. Vainerman, Finite quantum groupoids and their applications, New Directions
in Hopf algebras 43 (2002) 211--262
\bibitem{PS}P. Schauenburg, Hopf Algebra Extensions and Monoidal Categories, New Dir. Hopf Alg. 43 (2002)
\bibitem{PS2}P. Schauenburg, Computing Higher Frobenius-Schur Indicators in Fusion Categories Constructed from Inclusions of Finite Groups, Pacific J. Math. 280 (2016) 177--201
\bibitem{PS3}P. Schauenburg, Hopf Bimodules, Coquasibialgebras, and an Exact Sequence of Kac, Advances in Mathematics 165 (2002) 194–-263
\bibitem{ENO}P. Etingof, D. Nikshych and V. Ostrik, On fusion categories, Annals of Mathematics 162 (2005) 581--642
\bibitem{ENO2}P. Etingof, D. Nikshych and V. Ostrik, Weakly group-theoretical and solvable fusion categories, Advances in Mathematics 226(1) 176--205
\bibitem{EGNO}P. Etingof, S. Gelaki, D. Nikshych and V. Ostrik, Tensor Categories, Mathematical Surveys and Monographs 205 (2010)
\bibitem{Nat}S. Natale, Frobenius–Schur indicators for a class of fusion categories, Pacific J. Math. 221 (2005) 353--377,doi:10.2140/pjm.2005.221.353
\bibitem{BB}B. Bartlett, Categorical Aspects of Topological Quantum Field Theories, arXiv:math/0512103 [math.QA]
\bibitem{MS}M. Mignard and P. Schauenburg, Modular categories are not determined by their modular data, arXiv:1708.02796 [math]
\bibitem{Be}E. Beggs, Making non-trivially associated tensor categories from left coset representatives, J. Pure. App. Alg. 177 (2003) 5--41
\bibitem{Mol}R. Molnar, Semi-Direct Products of Hopf Algebras, J. Alg. 47 (1977) 29--51
\bibitem{Mom}J.M. Mombelli, Module categories over pointed Hopf algebras, Mathematische Zeitschrift 266 (2010) 319–-344 
\bibitem{Mom2}J.M. Mombelli, Representations of tensor categories coming from quantum linear spaces, J. Lond. Math. Soc. (2) 83 (2011) 19-–35
\bibitem{BDSV}B. Bartlett, C. Douglas, C. Schommer-Pries and J. Vicary, Modular categories as representations of the 3-dimensional bordism 2-category, arXiv:1509.06811 [math.AT]
\bibitem{FS}J. Fuchs and C. Schweigert, Category theory for conformal boundary conditions, Fields Institute Communications 39 (2003) 25--71
\bibitem{KM1}J. Klim and S. Majid, Hopf quasigroups and the algebraic 7-sphere, Journal of Algebra 323 (2010), doi:10.1016/j.jalgebra.2010.03.011
\bibitem{KM2}J. Klim and S. Majid, Bicrossproduct Hopf quasigroups, Comment. Math. Univ. Carolin. 51 (2010) 287–-304
\bibitem{Os2}V. Ostrik, Module categories over the Drinfeld double of a finite group, International Mathematics Research Notices 27 (2003) 1507–-1520, doi:10.1155/S1073792803205079
\bibitem{XGW1}X. G. Wen, Topological Orders in Rigid States, International Journal of Modern Physics B Vol. 04 (1990) 239--271 
\bibitem{Reut}D. Reutter, Higher linear algebra in topology and quantum information theory, Oxford DPhil thesis (2019)
\bibitem{DR}C. Douglas and D. Reutter, Fusion 2-categories and a state-sum invariant for 4-manifolds, arXiv:1812.11933 [math.QA]
\end{thebibliography}
